Pixelis: Reasoning in Pixels, from Seeing to Acting

Most vision-language systems are static observers: they describe pixels, do not act, and cannot safely improve under shift. This passivity limits generalizable, physically grounded visual intelligence. Learning through action, not static description, is essential beyond curated data. We present Pixelis, a pixel-space agent that operates directly on images and videos via a compact set of executable operations (zoom/crop, segment, track, OCR, temporal localization) and learns from its consequences. Pixelis trains in three phases: (1) Supervised Fine-Tuning learns a pixel-tool grammar from Chain-of-Thought-Action traces with a masked imitation loss that upweights operation/argument tokens and auxiliary heads to stabilize pixel-grounded arguments; (2) Curiosity-Coherence Reward Fine-Tuning optimizes a dual-drive objective marrying prediction-error curiosity with adjacent-step coherence and a mild efficiency prior under a KL anchor, yielding short, valid, structured toolchains; (3) Pixel Test-Time RL performs label-free adaptation by retrieving neighbors, voting over complete trajectories rather than answers, and updating toward short, high-fidelity exemplars while constraining drift with a KL-to-EMA safety control. Across six public image and video benchmarks, Pixelis yields consistent improvements: the average relative gain is +4.08% over the same 8B baseline (peaking at +6.03% on VSI-Bench), computed as (ours-baseline)/baseline, while producing shorter, auditable toolchains and maintaining in-corridor KL during test-time learning. Acting within pixels, rather than abstract tokens, grounds multimodal perception in the physical world, linking visual reasoning with actionable outcomes, and enables embodied adaptation without external feedback.

==> figures/figures.tex <==
\begin{table}[t]
\centering
\caption{\textbf{Framework comparison across benchmarks.} 95\% CIs in parentheses.}
\label{tab:framework_comp}
\resizebox{\linewidth}{!}{
\begin{tabular}{lccccccc}
\toprule
Model & Acc (\%) & IoU & CER (\%) & MOTA & RCS & AE & GC \\
\midrule
SFT-only                  & 58.1 & 0.62 & 5.9 & 0.55 & 0.33 & 0.71 & 0.68 \\
SFT+TTRL                  & 61.4 & 0.64 & 5.5 & 0.57 & 0.39 & 0.76 & 0.71 \\
SFT+RFT                   & 72.6 & 0.80 & 2.7 & 0.73 & 0.56 & 0.88 & 0.85 \\
\textbf{SFT+RFT+TTRL (ours)} & \textbf{76.9} & \textbf{0.83} & \textbf{2.3} & \textbf{0.78} & \textbf{0.62} & \textbf{0.92} & \textbf{0.89} \\
\bottomrule
\end{tabular}}
\end{table}

\begin{table}[t]
\centering
\caption{\textbf{Framework comparison across benchmarks.} 95\% CIs in parentheses.}
\label{tab:framework_comp}
\resizebox{\linewidth}{!}{
\begin{tabular}{lccccccc}
\toprule
Model & Acc (\%) & IoU & CER (\%) & MOTA & RCS & AE & GC \\
\midrule
SFT-only                  & 58.1 & 0.62 & 5.9 & 0.55 & 0.33 & 0.71 & 0.68 \\
SFT+TTRL                  & 61.4 & 0.64 & 5.5 & 0.57 & 0.39 & 0.76 & 0.71 \\
SFT+RFT                   & 72.6 & 0.80 & 2.7 & 0.73 & 0.56 & 0.88 & 0.85 \\
\textbf{SFT+RFT+TTRL (ours)} & \textbf{76.9} & \textbf{0.83} & \textbf{2.3} & \textbf{0.78} & \textbf{0.62} & \textbf{0.92} & \textbf{0.89} \\
\bottomrule
\end{tabular}}
\end{table}

\begin{table}[t]
\centering
\caption{\textbf{RQ1 ablations.} Best in bold.}
\label{tab:ablation_results}
\resizebox{\linewidth}{!}{
\begin{tabular}{lcccccccc}
\toprule
Variant & Acc (\%) & IoU & CER (\%) & MOTA & RCS & AE & GC & RaCPR \\
\midrule
RFT-Base ($R_{\text{final}}{+}R_{\text{pen}}$) & 63.5 & 0.72 & 4.9 & 0.61 & 0.42 & 0.79 & 0.81 & 0.55 \\
RFT-Curiosity ($+R_{\text{cur}}$)              & 68.9 & 0.76 & 3.6 & 0.66 & 0.47 & 0.84 & 0.83 & 0.61 \\
RFT-Coherence ($+R_{\text{coh}}$)               & 71.0 & 0.78 & 3.1 & 0.69 & 0.54 & 0.86 & 0.84 & 0.64 \\
\textbf{RFT-Full} ($+R_{\text{cur}}{+}R_{\text{coh}}{+}R_{\text{pen}}$) & \textbf{75.8} & \textbf{0.82} & \textbf{2.6} & \textbf{0.77} & \textbf{0.62} & \textbf{0.91} & \textbf{0.89} & \textbf{0.72} \\
\bottomrule
\end{tabular}}
\end{table}
